Contrastive Diffuser: Planning Towards High Return States via Contrastive Learning

The performance of offline reinforcement learning (RL) is sensitive to the proportion of high-return trajectories in the offline dataset. However, in many simulation environments and real-world scenarios, there are large ratios of low-return trajectories rather than high-return trajectories, which makes learning an efficient policy challenging. In this paper, we propose a method called Contrastive Diffuser (CDiffuser) to make full use of low-return trajectories and improve the performance of offline RL algorithms. Specifically, CDiffuser groups the states of trajectories in the offline dataset into high-return states and low-return states and treats them as positive and negative samples correspondingly. Then, it designs a contrastive mechanism to pull the trajectory of an agent toward high-return states and push them away from low-return states. Through the contrast mechanism, trajectories with low returns can serve as negative examples for policy learning, guiding the agent to avoid areas associated with low returns and achieve better performance. Experiments on 14 commonly used D4RL benchmarks demonstrate the effectiveness of our proposed method. Our code is publicly available at \url{https://anonymous.4open.science/r/CDiffuser}.

==> papers/0-abs-old.tex <==
\begin{abstract}
\lt{The performance of offline reinforcement learning (RL) is constrained by the proportion of high-return trajectories in the offline dataset. However, in many simulation environments and real-world scenarios, there are large ratios of low-return trajectories rather than high-return trajectories, which makes learning an efficient policy from these cases much challenging. In this paper, we propose a method called Contrastive Diffuser (CDiffuser), which devises a contrastive mechanism 
}

% Applying diffusion models in reinforcement learning for long-term planning has gained much attention recently. Several diffusion-based methods have successfully leveraged the modeling capabilities of diffusion for arbitrary distributions. These methods generate subsequent trajectories for planning and have demonstrated significant improvement.
% However, these methods are limited by their plain base distributions and their overlooking of the diversity of samples, in which different states have different returns.
% They simply leverage diffusion to learn the distribution of offline dataset, generate the trajectories whose states share the same distribution with the offline dataset. As a result, the probability of these models reaching the high-return states is largely dependent on the dataset distribution. Even equipped with the guidance model, the performance is still suppressed. To address these limitations, in this paper, we propose a novel method called CDiffuser, which devises a return contrast mechanism to pull the states in generated trajectories towards high-return states while pushing them away from low-return states to improve the base distribution. Experiments on 14 commonly used D4RL benchmarks demonstrate the effectiveness of our proposed method. Our code is publicly available at \url{https://anonymous.4open.science/r/CDiffuser}.

%Conditional diffusion models have made significant advances in many fields, which drives many reinforcement learning (RL) works view decision-making as a sequence generative problem and adopt diffusion models for action prediction. Despite the success of these methods in effectively modeling the underlying distribution, the biased learning has not been investigated yet.
% Besides, we observe that the existing methods based on classifier-guided diffusion models have an inherent flaw, which is that the un-biased learning of dataset distribution is actually working against the guidance.
% different states often possess different returns, which can be interpreted as distinct potentials of different states. Noticing this, inspired by contrastive learning, we propose Contrastive Diffuser, which is capable of learning the original data distribution while is also to planning towards states with higher returns by training biased towards high-return states. 
% Experiments on nine commonly used reinforcement learning tasks demonstrate the effectiveness of our approach over baseline algorithms. Our code will be public after the paper is reviewed.

% Diffusion models have made significant advances in many fields, which drives many reinforcement learning (RL) works to view decision-making as a sequence generative problem and adopt diffusion models for action prediction. Despite the success of these methods in effectively modeling the underlying distribution, we observe that the existing methods based on diffusion models have an inherent flaw, which is that the unbiased learning of the dataset distribution is actually working against the guidance by flattening the guidance distribution to a uniformed distribution over samples in the dataset. Noticing this, inspired by contrastive learning, we propose Contrastive Diffuser, a novel diffusion framework capable of learning the data distribution while also planning towards states with higher returns by training biased towards high-return states. Experiments on nine commonly used reinforcement learning tasks demonstrate the effectiveness of our approach over baseline algorithms. 
%Our code will be  made public after the paper is reviewed.

\end{abstract}


==> papers/1-intro-mod.tex <==
% \vspace{-20pt}
\section{Introduction}
% \longting{the intro should be major revised, the PIPELINE of intro:
% (1) what is offline RL, what relation between reward and offline RL;
% (2) How previous methods of different groups address offline RL problem? why they can not obtain high reward? e.g., without fully take use of samples in data?
% (3) how we address offline RL? why our solution will work;
% (4) experiment results demonstrates....
% (5) summary the contribution}

% As a significant branch of reinforcement learning (RL), o

\label{sec:intro}
Offline reinforcement learning (offline RL)~\cite{levine2020offline,prudencio2023survey} is a significant branch of reinforcement learning, where an agent is trained on pre-collected offline datasets and is evaluated online.
% and tested by deploying to interact with the environment. 
Since offline RL avoids potential risks from interacting with the environment during policy learning, it has broad applications in numerous real-world scenarios, 
% Since offline RL avoids the potential risks associated with interacting with the environment during policy learning, it has broad applications in numerous real-world scenarios, 
like commercial recommendation~\cite{xiao2021general}, health care~\cite{fatemi2022semi}, dialog~\cite{jaques2020human}, and autonomous driving~\cite{shi2021offline}. 

% Despite that, learning from static offline datasets brings extrapolation errors in offline RL, causing inaccurate value estimations on out-of-distribution (OOD) actions. 
% Due to their ability to model arbitrary distributions, using diffusion models to fit the entire dataset can effectively tackle these problems. A common approach is to utilize diffusion for long-term planning \cite{ajay2023is,janner2022planning}. Specifically, these methods leverage the diffusion model to generate subsequent trajectories, which include state-action pairs in a period of future. 
% \lt{Recently, some offline RL methods \cite{ajay2023is,janner2022planning} have incorporated diffusion for long-term planning, showcasing effectiveness and attracting considerable attention. Given the state of the current step, these methods depend on the diffusion model to generate the subsequent trajectories, and further apply the classifier guidance~\cite{dhariwal2021diffusion} to obtain the high-return trajectory, which contains the action response to the state. In training, the diffusion model is optimized by the mean-square-error of action and state in the generated sub-trajectories and the trajectories in the offline dataset, the classifier guidance model is optimized by the mean-square-error of the predicted return and the return in the offline dataset. }
% \lt{Since the decision-making process of these methods is dependent on the diffusion model and the classifier guidance model, and both of them are trained by the trajectories in the offline dataset, 

% \lt{}

\shanyx{Recently, some offline RL methods have incorporated diffusion for long-term planning, showcasing effectiveness and attracting considerable attention.
Taking advantages of diffusion models \cite{songdenoising, song2020denoising, ho2020denoising}, they generalize the distribution of the offline dataset and enhance the performance significantly. Despite the successes diffusion-based RL methods have achieved, their performance is still suppressed by the insufficient expert data in many scenarios~\cite{}. Besides, previous works~\cite{} regularize the discrepancy between the learned policy and behavior policy, making them highly sensitive to the sub-optimal demonstrations~\cite{yue2022boosting,wang2022diffusion,chen2023score}. For instance, as is shown in \cref{fig:intro} (a), the return of trajectories provided by the offline dataset of Maze2e-umaze-v1 are mostly concentrated on low-return area. Furthermore, such a lack of expert data can occur in many real-world scenarios, such as autonomous driving and medical diagnosis, achieving excellent performance with limited expert demonstrations remains a challenge for offline RL methods.



Take the goal-reaching toy model in \cref{fig:intro} as an example, in which the agent is supposed to reach a fixed goal position from a fixed  
start point. As is shown in \cref{fig:intro} (b), 

\sout{Moreover, in many real-world scenarios , rewards are only given when a certain condition is achieved, which also makes the number of high-return trajectories limited. } \shanyx{We are focusing on the lack of expert trajs, not lack of reward feedbacks} Therefore, 
% Although many works have been proposed to tackle these problems by augmenting expert data~\cite{ada2023diffusion}, the lack of expert data poses a challenge in reproducing reliable demonstrations. Instead, we proposed to make better use of the small proportion of real expert demonstrations in dataset.
}


\lt{
% However, owing to being trained with the offline data, the performance of offline RL methods is highly dependent on the proportion of the high-return trajectories in the offline dataset. 
However, the performance of offline RL methods highly depends on the proportion of the high-return trajectories in the offline dataset.
% , since they are trained with the offline data. 
When the dataset contains a large proportion of high-return trajectories, as it is presented in Figure \ref{fig:intro} (b), offline RL methods can easily learn the pattern of high-return trajectories such that they can achieve excellent performance when interacting with the environment.
% When the dataset contains a large proportion of high-return trajectories which offers a good pattern for offline RL methods to learn, they can easily achieve excellent performance when interacting with the environment after training,
% , as the high-return trajectories offer a good pattern for models to learn. .
In contrast, when the dataset has limited high-return trajectories, as it is presented in Figure \ref{fig:intro} (c), offline RL methods struggle to learn a good pattern from the dataset to achieve good returns.
% When high-return trajectories are limited in the dataset, the policies trained by the offline dataset struggle to achieve good returns, as it is presented in Figure \ref{fig:intro} (c).
Unfortunately, the issue of limited high-return trajectories commonly exists in both simulation environments and real-world scenarios. As it is illustrated in Figure \ref{fig:intro} (a), we visualize the probability density of trajectories' returns in Maze2d. The high-return trajectories are limited, in which the returns of most trajectories are located around 0.
% most trajectories are low-return. 
% Similarly, i


In real-world scenarios such as autonomous driving, and medical diagnosis, rewards are only given when a certain condition is achieved, which also makes the number of high-return trajectories limited. Therefore, achieving excellent performance in these scenarios remains a challenge for offline RL methods.}

\begin{figure*}
    

    \centering
    \includegraphics[width=1\textwidth]{figs/intro.pdf}

    \caption{Comparison of different distributions: (a) The dataset distribution; (b) The base distribution; (c) The distribution of classifier guide sampling; (d) The improved base distribution; (e) The improved distribution of classifier guide sampling.
    Each scatter in sub-figure represents a two-dimensional state, and the color of each scatter denotes the corresponding return.
    }
    \vspace{-10pt}
    \label{fig:intro}

\end{figure*}


% there are many cases in which high-return trajectories are insufficient. For instance, in autonomous driving, the car only receives a reward when it safely reaches its destination, and during the driving process, if there are no significant events (such as collisions or reaching intermediate goals), rewards are very insufficient. Similarly, in RL-assisted medical diagnosis, rewards are only given when the patient recovers, with no immediate feedback during the intermediate diagnosis and treatment processes. In some simulation environments such as Maze2d, the number of high-return trajectories is also limited as illustrated in Figure \ref{fig:intro} (d). All of these cases make it difficult for many offline RL methods to learn.
% Therefore, achieving excellent performance in these scenarios remains a challenge.
% How to fully utilize the limited high-return trajectories to achieve excellent performance is a challenge for many offline reinforcement learning methods. 


\lt{
Although high-return trajectories are limited in some offline datasets, there are abundant low-return trajectories. 
Notably, few works consider developing techniques to make full use of low-return trajectories.
% these two kinds of trajectories.
% We assume low-return
% Although high-return trajectories are sparse in offline datasets, there are abundant low-return trajectories, but they are not fully utilized by previous works.
As these low-return trajectories indicate potential areas where agents might obtain low returns,
% . Generally speaking, if 
We assume that if an agent achieves relatively high returns during its interactions with the environment, the trajectories generated during the interaction should maintain some differences from the low-return trajectories in the offline dataset. 
As illustrated in Figure \ref{fig:intro} (d), the trajectory of success to the goal position has a clear boundary from the low-return trajectories in the blue part.
Therefore, as it is illustrated in Figure \ref{fig:intro} (e), 
one promising solution to enable offline RL algorithms to achieve good returns is taking advantage of the differences between high-return and low-return trajectories: keeping the trajectory of the agent close to high-return trajectories, and away from low-return trajectories. 

% To achieve this goal, we need to address two issues: (1) what techniques to adopt; (2) which attributes of the trajectory to apply the techniques to. For the first issue, 
In RL domain, there are no mature techniques to pull the trajectories of an agent toward high-return trajectories and push them away from low-return trajectories. Fortunately, in the light of contrastive learning,
% there is an analogous case: contrastive learning,
a technique that aims to bring 
a given sample closer to positive (i.e., similar) samples and farther from negative (i.e., dissimilar) samples, we propose to treat high-return trajectories as positive samples and low-return trajectories as negative samples, and leverage contrastive learning to pull the trajectories toward high-return trajectories and push them away from low-return trajectories. 

!!!!!For the second issue, since states are an important part of the trajectories, reflecting the process of the agent interacting with the environment, we can apply the conservative mechanism to the states.

Considering some diffusion-based RL methods generate subsequent trajectories for planning, which contains an abundant number of states for contrasting, we build our method based on the states generated by those diffusion-based RL methods and propose a method called \textbf{Contrastive Diffuser} (\textbf{CDiffuser}). Specifically, we group the states of the trajectories in the offline dataset into high-return states and low-return states in a soft manner. Then, we learn a diffusion-based trajectory generation model to generate the trajectories whose states are constrained by contrastive learning to keep close to the high-return states and away from the low-return states.
Different from the previous works~\citep{qiu2022contrastive,laskin2020curl,yuan2022robust,agarwal2020contrastive} which leverage CL for the representation learning in RL, we introduce CL here to constrain the trajectories of agents.  To evaluate the performance of CDiffuser, we conduct experiment on 12 D4RL~\citep{fu2020d4rl} benchmarks. The experiment results demonstrate that CDiffuser has superior performance.
}


Recently, some offline RL methods have incorporated diffusion for long-term planning, showcasing effectiveness and attracting considerable attention.
Taking advantages of diffusion models \cite{songdenoising, song2020denoising, ho2020denoising}, they generalize the distribution of the offline dataset and enhance the performance significantly. 
% Specifically, these methods leverage the diffusion model to learn a distribution resembling the distribution of the offline dataset (we the distribution as base distribution), and further perform classifier-guided sampling over the learned base distribution for high-return trajectories. The generated trajectories are composed of planned state-action pairs in a period of future, in which the actions are generated by aggregating the information from the states before and after themselves.
Specifically, these methods leverage the diffusion model to generate the distribution of the subsequent trajectory \sout{(we name this distribution as \textbf{the base distribution})}, and further apply the classifier guidance~\cite{dhariwal2021diffusion} \sout{over the base distribution} to obtain a high-return trajectory, which contains the actions to be taken. In this process, the state-action pairs in the generated trajectory carry the planned future information and act as a condition for decision-making. As a result, these methods achieve outstanding performance in many tasks.


\shanyx
{
Despite the successes diffusion-based RL methods have achieved, their performance is still suppressed by the insufficient expert data in many scenarios~\cite{}. Moreover, previous works~\cite{} regularize the discrepancy between the learned policy and behavior policy, making them highly sensitive to the sub-optimal demonstrations~\cite{yue2022boosting,wang2022diffusion,chen2023score}. Although many works have been proposed to tackle these problems by augmenting expert data~\cite{ada2023diffusion}, the lack of expert data poses a challenge in reproducing reliable demonstrations. Instead, we proposed to make better use of the small proportion of real expert demonstrations in dataset.
<recall figure1>
}

% high-return trajectories. The generated trajectories are composed of planned state-action pairs in a period of future, in which the actions are generated by aggregating the information from the states before and after themselves.



% generate the trajectories that conform to the distribution of the offline dataset, which can enhance the generalization of policy significantly. Specifically, 

% Taking advantages of diffusion models in modeling arbitrary distributions, these methods effectively 


% One of the most efficient groups of offline RL is the methods that apply diffusion for long-term planning \cite{ajay2023is, janner2022planning}. Taking advantages of diffusion models in modeling arbitrary distributions, these methods have gained much attention recently.


% A common strategy of offline RL involves using diffusion models for long-term planning due to their ability to model arbitrary distributions, as highlighted in previous works \cite{ajay2023is, janner2022planning}. Specifically, these methods leverage the diffusion model to generate a distribution resembling the distribution of the offline dataset (we the distribution as base distribution).




% % However, learning from static offline datasets in offline Reinforcement Learning (RL) leads to extrapolation errors, resulting in inaccurate value estimations for out-of-distribution (OOD) actions. 
% % \shanyx{Due to their ability to model arbitrary distributions, many works adopt diffusion models to fit the entire dataset and effectively regularize the policy training.}
% % To address these issues effectively, diffusion models, known for their ability to model arbitrary distributions, are employed. A common strategy involves using diffusion models for long-term planning, as highlighted in previous works \cite{ajay2023is, janner2022planning}. Specifically, these methods leverage the diffusion model to generate a distribution resembling the distribution of the offline dataset (we the distribution as base distribution). 

% Then, they sample the base distribution to obtain the subsequent trajectories, and apply the classifier-guided sampling to obtain the 



% generate 
% \shanyx{

% }


% future trajectories, encompassing state-action pairs over a period of time.



% %One of the efficient solutions for this issue is diffusion based RL \cite{} 

% % While offline RL obviates costly online explorations, restricting the policy learning on static offline datasets poses additional challenges, \shanyx{such as the out of distribution (OOD) problem~\cite{fujimoto2019off}.}  \shanyx{review}
% %Directly applying off-policy algorithms in offline scenarios comes with the extrapolation error problem~\cite{fujimoto2019off}, which can cause inaccurate value estimations on out-of-distribution (OOD) actions to accumulate during Bellman backup. Extrapolation errors are alleviated in previous studies by adding conservative priors, \textit{e.g.}, regularizing the policy~\cite{fujimoto2021minimalist,wu2019behavior} or penalizing the value estimations~\cite{kumar2020conservative,kostrikov2021offline}. However, such conservative updates may cause the learning policy trapped in local optima, especially when offline datasets are collected by a mixture of policies~\cite{wang2022diffusion}. Recently, diffusion models have been used in offline RL as a powerful policy class~\cite{pearce2023imitating,chi2023diffusion,ada2023diffusion,wang2022diffusion}.
% % \shanyx{to give actions only~\cite{wang2022diffusion,ece2023diffusion,chi2023diffusion} or predict actions and states in the future for a certain period~\cite{janner2022planning,ajay2023is}}.
% Due to their ability to model arbitrary distributions, using diffusion models to fit the entire dataset can effectively regularize the policy without concerning of lacking expressiveness. Among 
% diffusion-based offline RL methods, a common approach is to utilize diffusion for long-term planning \cite{ajay2023is,janner2022planning}. Specifically, these methods leverage the diffusion model to generate subsequent trajectories, which include state-action pairs in a period of future. 
% The generated trajectories carry the estimated future states and enrich the information for planning, therefore they enhance models to make better decisions to be taken in the environment. 
% \shanyx{These methods leverage diffusion to model the dataset distribution, and further perform classifier-guided sampling over the learned distribution (which we name as the unguided distribution) for high-return trajectories. The generated trajectories include planned state-action pairs in a period of future, thus implies a plan for the future of the model; while the classifier-guided sampling, leveraging this plan, achieves premeditated adjustments for agents.}
% % 讲了太多diffusion RL的内容
% % 外推误差、OOD不是重点
% % 删掉
% % Direct application of off-policy algorithms in
% % offline scenarios comes with the extrapolation error prob-
% % lem (Fujimoto et al., 2019), which can cause inaccurate
% % value estimations on out-of-distribution (OOD) actions to
% % accumulate during Bellman backup. Extrapolation errors
% % are alleviated in prior studies by adding conservative pri-
% % ors, e.g., regularizing the policy (Fujimoto & Gu, 2021; Wu
% % et al., 2019) or penalizing the value estimations (Kumar
% % et al., 2020; Kostrikov et al., 2021). However, such con-
% % servative updates may leave the learning policy trapped in
% % local optima, especially when offline datasets are collected
% % by a mixture of policies (Wang et al., 2022).


% % the worry about lacking expressiveness. \shanyx{Nevertheless, the former diffusion-based methods fails in long-horizon planning, which is the methods mentioned later can.}

% % \zhengbang{In the next paragraph, say the drawbacks of uniformly fitting the entire dataset.}

% % Many outstanding works have been proposed for offline RL in recent years, which could be grouped into short-term decision-making and long-horizon planing methods. The short-term decision making works~\cite{konda1999actor,schulman2017proximal,babaeizadeh2016reinforcement,schulman2015trust,chen2021decision,janner2021offline} are deigned to predict the action of current step, which are unable to perform long-horizon planning. Therefore, the \textit{short-sight} leads them to be easily stuck in local optima~\cite{zhou2022pac,zhai2022monte,lu2022provable}. 
% % On the contrary, the long-horizon planing methods~\cite{janner2022planning, ajay2023is} take advantages of diffusion models~\cite{song2020denoising,song2020score,ho2020denoising,sohl2015deep} and have the capability of long-term planning. Specifically, they train the diffusion model to generate future trajectories according to the distribution of the offline dataset, take the generated trajectory for long-term planing, and utilize a function called guidance to guide the agent to reach desired states (\ie, states with high returns) in an explicit or implicit manner.

% % explicit \cite{janner2022planning} or implicit guidance \cite{ajay2023is} to selectively generate desired behaviors \longting{take the suitable actions?}, \textit{e.g.}, with high returns.
% % especially when there is large number of low-return samples in offline dataset. 





% The generated subsequent trajectory 
% Obtaining the subsequent trajectory usually involves convolution operations, the action corresponding to current state in the generated trajectory is naturally the optimal action in theory, since the action is inferred from the perspective of future \zhengbang{not clear why it is the optimal action}.
% However, these methods have insufficient utilization of dataset distribution. 
% \shanyx{Consider a dataset distribution as is shown in \cref{fig:intro}(a), where the green circle indicates the direction of guidance.}

% However, these methods neglect the diversity of samples in offline datasets, in which different states have different returns. They simply leverage diffusion to learn the dataset distribution and generate the trajectories whose states share the same distribution with the offline dataset.

% However, existing methods introducing diffusion models are limited by their plain base distributions and their neglecting of the diversity of samples in offline datasets.
% The classifier-guided sampling process of these methods can be viewed as sampling from a weighted average of two distributions: the base distribution and the  distribution of the classifier guidance. 
% Their base distributions are highly close to the dataset distribution, which makes these methods sensitive to the proportions of suboptimal samples in the dataset\cite{yue2022boosting,wang2022diffusion,chen2023score}.
% % They simply leverage diffusion to learn the dataset distribution and generate the trajectories whose states share the same distribution with the offline dataset.
% % \shanyx{What should be done to high/low val states}
% As shown in \cref{fig:intro}, the base distribution (b), where the generated trajectories are samples from, is similar to the original distribution of the offline dataset (a), making the probability of sampling high-return states restricted if there are many low-return states in the dataset. 
% % Despite introducing guidance, a function that guides the agent to produce optimal\shanyx{} actions based on the results generated by diffusion,\shanyx{mark} there is no significant improvement,\shanyx{improvement seems confusing} as depicted in Figure \cref{fig:intro}(c). 
% Even with classifier guidance~\cite{dhariwal2021diffusion} techniques to enforce the generation towards the high-return area, the results remain unsatisfactory as depicted in \cref{fig:intro}(c). Although the sampling distribution is more concentrated within the guidance circle, there are still many samples spread over the entire low-return area, which may cause many low-return states in the generated trajectories.
% Intuitively, if constraining the base distribution to be close to the area with high-return states and away from the area with low-return states, like Figure \ref{fig:intro} (d), we would obtain better results under the guidance, like \cref{fig:intro}(e).



% \textbf{Version B}
% Among diffusion-based offline RL methods, a common approach is to utilize diffusion for long-term planning \zhengbang{cite}. Specifically, these methods leverage a guided sampling of a diffusion model to generate subsequent trajectories containing state-action pairs for planning. The guided sampling procedure can be viewed as sampling from a joint distribution of a guidance distribution and a base distribution. Note that the guidance distribution concentrates on the high return states provided by a rating function, \ie, states within the area marked by the circle in \cref{fig:intro} (a); the base distribution is an uniform distribution over the dataset learned by diffusion model as shown in \cref{fig:intro} (b). The joint distribution is shown in \cref{fig:intro} (c). 
% As can be observed, although the joint distribution does pay more attention on the high return states, due to the uniform base distribution, there are still a number of samples fall into the low return states.
% Intuitively, if we can improve the base distribution to close to the area with high-return states and away from the area with low-return states, like Figure \ref{fig:intro} (d), we would obtain better results like \cref{fig:intro}(e) under the guidance.




Considering contrastive learning (CL)~\cite{khosla2020supervised, yeh2022decoupled} 
is designed for pulling a sample towards similar samples and pushing it away from dissimilar samples, 
which is analogous to the case of pulling the states in the generated trajectory towards the high-return areas and away from low-return areas,
we introduce contrastive learning to diffusion-based RL methods and propose a novel method called \textbf{Contrastive Diffuser} (\textbf{CDiffuser}). Different from the previous works~\cite{qiu2022contrastive,laskin2020curl,yuan2022robust,agarwal2020contrastive} which leverage CL for the representation learning in RL, 
we introduce CL to improve the base distribution of diffusion-based RL method with contrastive mechanism.
Specifically, we group the states in the offline dataset into high-return states and low-return states in a soft manner. Then, we learn a diffusion-based trajectory generation model to generate the trajectories whose states are constrained by contrastive learning. In such manner, the base distribution (see \cref{fig:intro}(b)) is enhanced. 
As a result, the states in generated trajectories closely align with high-return states while staying away from low-return states.
% close to the positive sample and away from the negative sample, and the learning process is constrained with contrastive learning.
% our method composes of Trajectory Generation Module, Contrastive Module and Guidance Module.  The Trajectory Generation Module is designed for the long-term planning, which is implemented with diffusion. The Contrastive Module is designed to constrain the generated trajctories to high-return states. The Guidance Module is designed for guiding agent to take suitable actions. 
With the help of contrastive learning, CDiffuser generates better trajectories for planning.
% In that way, CDiffuser obtains better generated trajectory for planning.
 To evaluate the performance of CDiffuser, we conduct experiments on 14 D4RL benchmarks~\cite{fu2020d4rl}. The experiment results demonstrate that CDiffuser has superior performance.% compared to existing methods.



% \shanyx{
% Different from the previous works~\cite{qiu2022contrastive,laskin2020curl,yuan2022robust,agarwal2020contrastive} which leverage contrastive learning for better representation, we leverage contrastive learning to priori improve the base distribution, as is shown in \cref{fig:intro} (d). 
% Specifically, we perform contrastive learning to learn a distribution whose probability density is concentrated in high value areas, rather than a uniform distribution (on dataset samples) like Decision Diffuser and Diffuser.
% Firstly, according to the state values, states in the offline dataset are grouped into positive samples (high-value states) and negative samples (low-value states). To mitigate the costs associated with the erroneous classification of samples near the boundaries, we design a influence function for the soft manner of clustering for grouping. Further, the states from generated trajectories as well as the positive and negative samples are mapped into the same space for contrasting to improve the base distribution.  With the help of contrastive learning, CDiffuser generates better trajectories with high-value states, and performs ???? in planning tasks. The results  on 12 D4RL~\cite{fu2020d4rl} benchmarks and  analysis of CDiffuser  prove the ??? of CDiffuser.
% }


In summary, our contributions are: 
(\romannumeral 1) We propose a method called CDiffuser, which novelly improves the base distribution of diffusion-based RL methods and achieves outstanding performance, providing an innovative perspective of improving diffusion-based RL methods for the subsequent works.
% \todo{the base diffusion distribution} towards high-return \todo{areas}.
(\romannumeral 2) We perform contrastive learning over returns of states to improve the base distribution. To the best of our knowledge, our work is the first which notices the limitation of the base distribution, and the first which applies contrastive learning to enhance the base distribution for diffusion based RL methods.
(\romannumeral 3) Experiment results on 14 D4RL datasets demonstrate the outstanding performance of CDiffuser.
% , as well as the success of the guided \todo{ base distribution} learning provided by contrastive learning.

% adopts contrastive learning and is capable of generating biased trajectories towards the area of higher return states. (3) Experiments on D4RL datasets show that CDiffuser outperforms other baseline methods and further demonstrates the significance of the \textit{state-return} distribution in successful action prediction. (4) Thanks to the consideration of the \textit{state-return} distribution, CDiffuser is able to mitigate the out-of-distribution (OOD) problem as it intentionally encourages the agent to approach the high-potential state distribution, which is precisely in the distribution of collected dataset. 

% Noticing the aforementioned challenges while inspired by contrastive learning, we propose \textbf{CDiffuser}, which pays attention on $state-return$ distribution and adopt contrastive learning to bias the learning process towards high-return states while away from low-return states, thus guides the learning of trajectory generation and leverages the information present in the dataset more comprehensively.
% Specifically, we adopt a trajectory generation model based on diffusion models as the base model, while an auxiliary optimize object based on contrastive learning is further adopted to ensure that the predicted trajectories' states fall within the positive sample distribution as much as possible while avoiding the negative sample distribution. 
% Details of our model will be further detailed in \cref{sec:Methods}. Experiment results on nine commonly used benchmarks demonstrates that CDiffuser has the capability to guide the agent towards a state space characterized by higher returns, thus exhibiting superior performance compared to existing methods.

% In summary, our contributions are as follows: (1) We identify the shortcomings of existing diffusion-based RL methods and provide a practical solution. (2) We propose a novel diffusion-based RL method, CDiffuser, which adopts contrastive learning and is capable of generating biased trajectories towards the area of higher return states. (3) Experiments on D4RL datasets show that CDiffuser outperforms other baseline methods and further demonstrates the significance of the \textit{state-return} distribution in successful action prediction. (4) Thanks to the consideration of the \textit{state-return} distribution, CDiffuser is able to mitigate the out-of-distribution (OOD) problem as it intentionally encourages the agent to approach the high-potential state distribution, which is precisely in the distribution of collected dataset. 


==> papers/1-intro-old.tex <==
% \vspace{-20pt}
\section{Introduction}
% \longting{the intro should be major revised, the PIPELINE of intro:
% (1) what is offline RL, what relation between reward and offline RL;
% (2) How previous methods of different groups address offline RL problem? why they can not obtain high reward? e.g., without fully take use of samples in data?
% (3) how we address offline RL? why our solution will work;
% (4) experiment results demonstrates....
% (5) summary the contribution}

% As a significant branch of reinforcement learning (RL), o

\label{sec:intro}
Offline reinforcement learning (offline RL)~\citep{levine2020offline,prudencio2023survey} is a significant branch of reinforcement learning, where an agent is trained on pre-collected offline datasets and is evaluated online.
% and tested by deploying to interact with the environment. 
Since offline RL avoids potential risks from interacting with the environment during policy learning, it has broad applications in numerous real-world scenarios, 
% Since offline RL avoids the potential risks associated with interacting with the environment during policy learning, it has broad applications in numerous real-world scenarios, 
like commercial recommendation~\citep{xiao2021general}, health care~\citep{fatemi2022semi}, dialog~\citep{jaques2020human}, and autonomous driving~\citep{shi2021offline}. 

% Despite that, learning from static offline datasets brings extrapolation errors in offline RL, causing inaccurate value estimations on out-of-distribution (OOD) actions. 
% Due to their ability to model arbitrary distributions, using diffusion models to fit the entire dataset can effectively tackle these problems. A common approach is to utilize diffusion for long-term planning \cite{ajay2023is,janner2022planning}. Specifically, these methods leverage the diffusion model to generate subsequent trajectories, which include state-action pairs in a period of future. 
% \lt{Recently, some offline RL methods \cite{ajay2023is,janner2022planning} have incorporated diffusion for long-term planning, showcasing effectiveness and attracting considerable attention. Given the state of the current step, these methods depend on the diffusion model to generate the subsequent trajectories, and further apply the classifier guidance~\cite{dhariwal2021diffusion} to obtain the high-return trajectory, which contains the action response to the state. In training, the diffusion model is optimized by the mean-square-error of action and state in the generated sub-trajectories and the trajectories in the offline dataset, the classifier guidance model is optimized by the mean-square-error of the predicted return and the return in the offline dataset. }
% \lt{Since the decision-making process of these methods is dependent on the diffusion model and the classifier guidance model, and both of them are trained by the trajectories in the offline dataset, 

% \lt{}


\lt{
% However, owing to being trained with the offline data, the performance of offline RL methods is highly dependent on the proportion of the high-return trajectories in the offline dataset. 
However, the performance of offline RL methods highly depends on the proportion of the high-return trajectories in the offline dataset.
% , since they are trained with the offline data. 
When the dataset contains a large proportion of high-return trajectories, as it is presented in Figure \ref{fig:intro} (b), offline RL methods can easily learn the pattern of high-return trajectories such that they can achieve excellent performance when interacting with the environment.
% When the dataset contains a large proportion of high-return trajectories which offers a good pattern for offline RL methods to learn, they can easily achieve excellent performance when interacting with the environment after training,
% , as the high-return trajectories offer a good pattern for models to learn. .
In contrast, when the dataset has limited high-return trajectories, as it is presented in Figure \ref{fig:intro} (c), offline RL methods struggle to learn a good pattern from the dataset to achieve good returns.
% When high-return trajectories are limited in the dataset, the policies trained by the offline dataset struggle to achieve good returns, as it is presented in Figure \ref{fig:intro} (c).
Unfortunately, the issue of limited high-return trajectories commonly exists in both simulation environments and real-world scenarios. As it is illustrated in Figure \ref{fig:intro} (a), we visualize the probability density of trajectories' returns in Maze2d. We can observe that high-return trajectories are much limited.
% The high-return trajectories are limited, in which the returns of most trajectories are located around 0.
% most trajectories are low-return. 
% Similarly, i
% \shanyx{We focus on the lack of expert data, not sparse rewards}
In real-world scenarios such as autonomous driving, and medical diagnosis, rewards are only given when a certain condition is achieved, which also makes the number of high-return trajectories limited \cite{prudencio2023survey}. Therefore, achieving excellent performance in these scenarios remains a challenge for offline RL methods.}

\begin{figure*}
    

    \centering
    \includegraphics[width=1\textwidth]{figs/intro.pdf}

    \caption{(a) The probability density of trajectories’ returns in Maze2d; (b) The learned trajectory when high-return trajectories are abundant;  (c) The learned trajectory when high-return trajectories are limited; (d) The contrastive learning applied by previous RL models; (e) The example of our solution.
    }
    \label{fig:intro}
\end{figure*}


% there are many cases in which high-return trajectories are insufficient. For instance, in autonomous driving, the car only receives a reward when it safely reaches its destination, and during the driving process, if there are no significant events (such as collisions or reaching intermediate goals), rewards are very insufficient. Similarly, in RL-assisted medical diagnosis, rewards are only given when the patient recovers, with no immediate feedback during the intermediate diagnosis and treatment processes. In some simulation environments such as Maze2d, the number of high-return trajectories is also limited as illustrated in Figure \ref{fig:intro} (d). All of these cases make it difficult for many offline RL methods to learn.
% Therefore, achieving excellent performance in these scenarios remains a challenge.
% How to fully utilize the limited high-return trajectories to achieve excellent performance is a challenge for many offline reinforcement learning methods. 


\lt{
Although high-return trajectories are limited in some cases, there are abundant low-return trajectories. 
Notably, few works consider developing techniques to make full use of low-return trajectories.
% these two kinds of trajectories.
% We assume low-return
% Although high-return trajectories are sparse in offline datasets, there are abundant low-return trajectories, but they are not fully utilized by previous works.
As states in those low-return trajectories indicate potential areas where agents might obtain low returns,
% . Generally speaking, if 
We assume that if an agent achieves relatively high returns during its interactions with the environment, the trajectories generated during the interaction should maintain some different states from the low-return trajectories in the offline dataset. 
As illustrated in Figure \ref{fig:intro} (a), some states (marked in blue dot) in the trajectories that can reach the goal position
% in the trajectory of success to the goal position 
have a clear boundary from the ones in low-return trajectories.
Therefore, as it is illustrated in Figure \ref{fig:intro} (e), 
one promising solution to enable offline RL algorithms to achieve good returns is taking advantage of the state differences between high-return and low-return trajectories: keeping the states in the agent's trajectory close to high-return states, and away from low-return states. 

% To achieve this goal, we need to address two issues: (1) what techniques to adopt; (2) which attributes of the trajectory to apply the techniques to. For the first issue, 
However, in RL domain, there are no mature techniques to pull the states of a trajectory toward high-return states and push them away from low-return states, to the best of our knowledge. Fortunately, in the light of contrastive learning,
% there is an analogous case: contrastive learning,
a technique that aims to bring 
a given sample closer to positive (i.e., similar) samples and farther from negative (i.e., dissimilar) samples, we propose to treat high-return states in trajectories of offline dataset as positive samples and the ones with low return as negative samples, and leverage contrastive learning to pull the states toward high-return states and push them away from low-return states. It is worth noting that, unlike previous contrastive learning based works  ~\citep{qiu2022contrastive,laskin2020curl,yuan2022robust,agarwal2020contrastive}, which apply contrastive learning to constrain the states of the same trajectory to similar representation, and the states of different trajectories to different representation, as it is illustrated in Figure \ref{fig:intro} (c). We aim to \textbf{use contrastive learning to constrain policy toward high-return states and away from low-return states} (Figure \ref{fig:intro} (d)).  
Furthermore, the criteria for distinguishing positive and negative samples here are based on the returns of the states rather than the categories of the samples.


% With the contrastive mechanism, low return trajectories could be make full use of and  the agent is supposed to be constrained toward the high-return states and ultimately obtains a high reward. 
Through the contrast mechanism, trajectories with low returns can serve as negative examples for policy learning, guiding the agent to avoid areas associated with low returns. Additionally, with the guidance of high-return states, the agent ultimately achieves high returns.
 % could obtain a better policy and 
% However, the paradox lies in the fact that the states used for contrasting depend on the policy, and the contrasting among states is designed for better policy.
However, ordinary states are feedback from the environment rather than generated by the model, applying contrastive mechanisms to these states has little help in policy optimization.
% !!!!!For the second issue, since states are an important part of the trajectories, reflecting the process of the agent interacting with the environment, we can apply the conservative mechanism to the states.
Considering some diffusion-based RL methods generate subsequent trajectories for planning \citep{janner2022planning,ajay2023is}, in which abundant states are generated by policy model,
% and the states in the generated trajectories could be applied for the contrasting state and offering the information of high-return area for decision making, 
% which contains an abundant number of states in the generated subsequent trajectories.
% for contrasting, 
we build our method based on the states generated by those diffusion-based RL methods and propose a method called \textbf{Contrastive Diffuser} (\textbf{CDiffuser}). Specifically, we first group the states of the trajectories in the offline dataset into high-return states and low-return states in a soft manner. 
Then, we learn a diffusion-based trajectory generation model to generate the subsequent trajectories, and apply a contrastive mechanism to the states of the generated trajectories to pull them toward the high-return states and push them away from the low-return states in the offline dataset.
% whose states are constrained by contrastive learning to keep close to the high-return states and away from the low-return states.
% Different from the previous works~\citep{qiu2022contrastive,laskin2020curl,yuan2022robust,agarwal2020contrastive} which leverage CL for the representation learning in RL, we introduce CL here to constrain the trajectories of agents. 
With the contrastive mechanism constrained states for planning, the agent makes better decisions towards the high-return states.
To evaluate the performance of CDiffuser, we conduct experiment on 14 D4RL~\citep{fu2020d4rl} benchmarks. The experiment results demonstrate that CDiffuser has superior performance.

In summary, our contributions are: 
(\romannumeral 1) We propose a method called CDiffuser, which takes the advantage of low-return trajectories by pulling the states in trajectories toward to high-return states and pushing away from low-return states.
% novelly improves the base distribution of diffusion-based RL methods and achieves outstanding performance, providing an innovative perspective of improving diffusion-based RL methods for the subsequent works.
% \todo{the base diffusion distribution} towards high-return \todo{areas}.
(\romannumeral 2) We perform contrastive learning for pulling the states in trajectories toward to high-return states and pushing away from low-return states. To the best of our knowledge, our work is the first which apply contrastive learning to enhance the policy learning.
% (\romannumeral 2) We perform contrastive learning over returns of states to improve the base distribution. To the best of our knowledge, our work is the first which notices the limitation of the base distribution, and the first which applies contrastive learning to enhance the base distribution for diffusion based RL methods.
(\romannumeral 3) Experiment results on 14 D4RL datasets demonstrate the outstanding performance of CDiffuser.

}


% Recently, some offline RL methods have incorporated diffusion for long-term planning, showcasing effectiveness and attracting considerable attention.
% Taking advantages of diffusion models \cite{songdenoising, song2020denoising, ho2020denoising}, they generalize the distribution of the offline dataset and enhance the performance significantly. 
% Specifically, these methods leverage the diffusion model to learn a distribution resembling the distribution of the offline dataset (we the distribution as base distribution), and further perform classifier-guided sampling over the learned base distribution for high-return trajectories. The generated trajectories are composed of planned state-action pairs in a period of future, in which the actions are generated by aggregating the information from the states before and after themselves.
% Specifically, these methods leverage the diffusion model to generate the distribution of the subsequent trajectory \sout{(we name this distribution as \textbf{the base distribution})}, and further apply the classifier guidance~\cite{dhariwal2021diffusion} \sout{over the base distribution} to obtain a high-return trajectory, which contains the actions to be taken. In this process, the state-action pairs in the generated trajectory carry the planned future information and act as a condition for decision-making. As a result, these methods achieve outstanding performance in many tasks.


% \shanyx
% {
% Despite the successes diffusion-based RL methods have achieved, their performance is still suppressed by the insufficient expert data in many scenarios~\cite{}. Moreover, previous works~\cite{} regularize the discrepancy between the learned policy and behavior policy, making them highly sensitive to the sub-optimal demonstrations~\cite{yue2022boosting,wang2022diffusion,chen2023score}. Although many works have been proposed to tackle these problems by augmenting expert data~\cite{ada2023diffusion}, the lack of expert data poses a challenge in reproducing reliable demonstrations. Instead, we proposed to make better use of the small proportion of real expert demonstrations in dataset.
% <recall figure1>
% }

% high-return trajectories. The generated trajectories are composed of planned state-action pairs in a period of future, in which the actions are generated by aggregating the information from the states before and after themselves.



% generate the trajectories that conform to the distribution of the offline dataset, which can enhance the generalization of policy significantly. Specifically, 

% Taking advantages of diffusion models in modeling arbitrary distributions, these methods effectively 


% One of the most efficient groups of offline RL is the methods that apply diffusion for long-term planning \cite{ajay2023is, janner2022planning}. Taking advantages of diffusion models in modeling arbitrary distributions, these methods have gained much attention recently.


% A common strategy of offline RL involves using diffusion models for long-term planning due to their ability to model arbitrary distributions, as highlighted in previous works \cite{ajay2023is, janner2022planning}. Specifically, these methods leverage the diffusion model to generate a distribution resembling the distribution of the offline dataset (we the distribution as base distribution).




% % However, learning from static offline datasets in offline Reinforcement Learning (RL) leads to extrapolation errors, resulting in inaccurate value estimations for out-of-distribution (OOD) actions. 
% % \shanyx{Due to their ability to model arbitrary distributions, many works adopt diffusion models to fit the entire dataset and effectively regularize the policy training.}
% % To address these issues effectively, diffusion models, known for their ability to model arbitrary distributions, are employed. A common strategy involves using diffusion models for long-term planning, as highlighted in previous works \cite{ajay2023is, janner2022planning}. Specifically, these methods leverage the diffusion model to generate a distribution resembling the distribution of the offline dataset (we the distribution as base distribution). 

% Then, they sample the base distribution to obtain the subsequent trajectories, and apply the classifier-guided sampling to obtain the 



% generate 
% \shanyx{

% }


% future trajectories, encompassing state-action pairs over a period of time.



% %One of the efficient solutions for this issue is diffusion based RL \cite{} 

% % While offline RL obviates costly online explorations, restricting the policy learning on static offline datasets poses additional challenges, \shanyx{such as the out of distribution (OOD) problem~\cite{fujimoto2019off}.}  \shanyx{review}
% %Directly applying off-policy algorithms in offline scenarios comes with the extrapolation error problem~\cite{fujimoto2019off}, which can cause inaccurate value estimations on out-of-distribution (OOD) actions to accumulate during Bellman backup. Extrapolation errors are alleviated in previous studies by adding conservative priors, \textit{e.g.}, regularizing the policy~\cite{fujimoto2021minimalist,wu2019behavior} or penalizing the value estimations~\cite{kumar2020conservative,kostrikov2021offline}. However, such conservative updates may cause the learning policy trapped in local optima, especially when offline datasets are collected by a mixture of policies~\cite{wang2022diffusion}. Recently, diffusion models have been used in offline RL as a powerful policy class~\cite{pearce2023imitating,chi2023diffusion,ada2023diffusion,wang2022diffusion}.
% % \shanyx{to give actions only~\cite{wang2022diffusion,ece2023diffusion,chi2023diffusion} or predict actions and states in the future for a certain period~\cite{janner2022planning,ajay2023is}}.
% Due to their ability to model arbitrary distributions, using diffusion models to fit the entire dataset can effectively regularize the policy without concerning of lacking expressiveness. Among 
% diffusion-based offline RL methods, a common approach is to utilize diffusion for long-term planning \cite{ajay2023is,janner2022planning}. Specifically, these methods leverage the diffusion model to generate subsequent trajectories, which include state-action pairs in a period of future. 
% The generated trajectories carry the estimated future states and enrich the information for planning, therefore they enhance models to make better decisions to be taken in the environment. 
% \shanyx{These methods leverage diffusion to model the dataset distribution, and further perform classifier-guided sampling over the learned distribution (which we name as the unguided distribution) for high-return trajectories. The generated trajectories include planned state-action pairs in a period of future, thus implies a plan for the future of the model; while the classifier-guided sampling, leveraging this plan, achieves premeditated adjustments for agents.}
% % 讲了太多diffusion RL的内容
% % 外推误差、OOD不是重点
% % 删掉
% % Direct application of off-policy algorithms in
% % offline scenarios comes with the extrapolation error prob-
% % lem (Fujimoto et al., 2019), which can cause inaccurate
% % value estimations on out-of-distribution (OOD) actions to
% % accumulate during Bellman backup. Extrapolation errors
% % are alleviated in prior studies by adding conservative pri-
% % ors, e.g., regularizing the policy (Fujimoto & Gu, 2021; Wu
% % et al., 2019) or penalizing the value estimations (Kumar
% % et al., 2020; Kostrikov et al., 2021). However, such con-
% % servative updates may leave the learning policy trapped in
% % local optima, especially when offline datasets are collected
% % by a mixture of policies (Wang et al., 2022).


% % the worry about lacking expressiveness. \shanyx{Nevertheless, the former diffusion-based methods fails in long-horizon planning, which is the methods mentioned later can.}

% % \zhengbang{In the next paragraph, say the drawbacks of uniformly fitting the entire dataset.}

% % Many outstanding works have been proposed for offline RL in recent years, which could be grouped into short-term decision-making and long-horizon planing methods. The short-term decision making works~\cite{konda1999actor,schulman2017proximal,babaeizadeh2016reinforcement,schulman2015trust,chen2021decision,janner2021offline} are deigned to predict the action of current step, which are unable to perform long-horizon planning. Therefore, the \textit{short-sight} leads them to be easily stuck in local optima~\cite{zhou2022pac,zhai2022monte,lu2022provable}. 
% % On the contrary, the long-horizon planing methods~\cite{janner2022planning, ajay2023is} take advantages of diffusion models~\cite{song2020denoising,song2020score,ho2020denoising,sohl2015deep} and have the capability of long-term planning. Specifically, they train the diffusion model to generate future trajectories according to the distribution of the offline dataset, take the generated trajectory for long-term planing, and utilize a function called guidance to guide the agent to reach desired states (\ie, states with high returns) in an explicit or implicit manner.

% % explicit \cite{janner2022planning} or implicit guidance \cite{ajay2023is} to selectively generate desired behaviors \longting{take the suitable actions?}, \textit{e.g.}, with high returns.
% % especially when there is large number of low-return samples in offline dataset. 





% The generated subsequent trajectory 
% Obtaining the subsequent trajectory usually involves convolution operations, the action corresponding to current state in the generated trajectory is naturally the optimal action in theory, since the action is inferred from the perspective of future \zhengbang{not clear why it is the optimal action}.
% However, these methods have insufficient utilization of dataset distribution. 
% \shanyx{Consider a dataset distribution as is shown in \cref{fig:intro}(a), where the green circle indicates the direction of guidance.}

% However, these methods neglect the diversity of samples in offline datasets, in which different states have different returns. They simply leverage diffusion to learn the dataset distribution and generate the trajectories whose states share the same distribution with the offline dataset.

% However, existing methods introducing diffusion models are limited by their plain base distributions and their neglecting of the diversity of samples in offline datasets.
% The classifier-guided sampling process of these methods can be viewed as sampling from a weighted average of two distributions: the base distribution and the  distribution of the classifier guidance. 
% Their base distributions are highly close to the dataset distribution, which makes these methods sensitive to the proportions of suboptimal samples in the dataset\cite{yue2022boosting,wang2022diffusion,chen2023score}.
% % They simply leverage diffusion to learn the dataset distribution and generate the trajectories whose states share the same distribution with the offline dataset.
% % \shanyx{What should be done to high/low val states}
% As shown in \cref{fig:intro}, the base distribution (b), where the generated trajectories are samples from, is similar to the original distribution of the offline dataset (a), making the probability of sampling high-return states restricted if there are many low-return states in the dataset. 
% % Despite introducing guidance, a function that guides the agent to produce optimal\shanyx{} actions based on the results generated by diffusion,\shanyx{mark} there is no significant improvement,\shanyx{improvement seems confusing} as depicted in Figure \cref{fig:intro}(c). 
% Even with classifier guidance~\cite{dhariwal2021diffusion} techniques to enforce the generation towards the high-return area, the results remain unsatisfactory as depicted in \cref{fig:intro}(c). Although the sampling distribution is more concentrated within the guidance circle, there are still many samples spread over the entire low-return area, which may cause many low-return states in the generated trajectories.
% Intuitively, if constraining the base distribution to be close to the area with high-return states and away from the area with low-return states, like Figure \ref{fig:intro} (d), we would obtain better results under the guidance, like \cref{fig:intro}(e).



% \textbf{Version B}
% Among diffusion-based offline RL methods, a common approach is to utilize diffusion for long-term planning \zhengbang{cite}. Specifically, these methods leverage a guided sampling of a diffusion model to generate subsequent trajectories containing state-action pairs for planning. The guided sampling procedure can be viewed as sampling from a joint distribution of a guidance distribution and a base distribution. Note that the guidance distribution concentrates on the high return states provided by a rating function, \ie, states within the area marked by the circle in \cref{fig:intro} (a); the base distribution is an uniform distribution over the dataset learned by diffusion model as shown in \cref{fig:intro} (b). The joint distribution is shown in \cref{fig:intro} (c). 
% As can be observed, although the joint distribution does pay more attention on the high return states, due to the uniform base distribution, there are still a number of samples fall into the low return states.
% Intuitively, if we can improve the base distribution to close to the area with high-return states and away from the area with low-return states, like Figure \ref{fig:intro} (d), we would obtain better results like \cref{fig:intro}(e) under the guidance.




% Considering contrastive learning (CL)~\cite{khosla2020supervised, yeh2022decoupled} 
% is designed for pulling a sample towards similar samples and pushing it away from dissimilar samples, 
% which is analogous to the case of pulling the states in the generated trajectory towards the high-return areas and away from low-return areas,
% we introduce contrastive learning to diffusion-based RL methods and propose a novel method called \textbf{Contrastive Diffuser} (\textbf{CDiffuser}). Different from the previous works~\cite{qiu2022contrastive,laskin2020curl,yuan2022robust,agarwal2020contrastive} which leverage CL for the representation learning in RL, 
% we introduce CL to improve the base distribution of diffusion-based RL method with contrastive mechanism.
% Specifically, we group the states in the offline dataset into high-return states and low-return states in a soft manner. Then, we learn a diffusion-based trajectory generation model to generate the trajectories whose states are constrained by contrastive learning. In such manner, the base distribution (see \cref{fig:intro}(b)) is enhanced. 
% As a result, the states in generated trajectories closely align with high-return states while staying away from low-return states.
% % close to the positive sample and away from the negative sample, and the learning process is constrained with contrastive learning.
% % our method composes of Trajectory Generation Module, Contrastive Module and Guidance Module.  The Trajectory Generation Module is designed for the long-term planning, which is implemented with diffusion. The Contrastive Module is designed to constrain the generated trajctories to high-return states. The Guidance Module is designed for guiding agent to take suitable actions. 
% With the help of contrastive learning, CDiffuser generates better trajectories for planning.
% % In that way, CDiffuser obtains better generated trajectory for planning.
%  To evaluate the performance of CDiffuser, we conduct experiments on 14 D4RL benchmarks~\cite{fu2020d4rl}. The experiment results demonstrate that CDiffuser has superior performance.% compared to existing methods.



% \shanyx{
% Different from the previous works~\cite{qiu2022contrastive,laskin2020curl,yuan2022robust,agarwal2020contrastive} which leverage contrastive learning for better representation, we leverage contrastive learning to priori improve the base distribution, as is shown in \cref{fig:intro} (d). 
% Specifically, we perform contrastive learning to learn a distribution whose probability density is concentrated in high value areas, rather than a uniform distribution (on dataset samples) like Decision Diffuser and Diffuser.
% Firstly, according to the state values, states in the offline dataset are grouped into positive samples (high-value states) and negative samples (low-value states). To mitigate the costs associated with the erroneous classification of samples near the boundaries, we design a influence function for the soft manner of clustering for grouping. Further, the states from generated trajectories as well as the positive and negative samples are mapped into the same space for contrasting to improve the base distribution.  With the help of contrastive learning, CDiffuser generates better trajectories with high-value states, and performs ???? in planning tasks. The results  on 12 D4RL~\cite{fu2020d4rl} benchmarks and  analysis of CDiffuser  prove the ??? of CDiffuser.
% }


% In summary, our contributions are: 
% (\romannumeral 1) We propose a method called CDiffuser, which novelly improves the base distribution of diffusion-based RL methods and achieves outstanding performance, providing an innovative perspective of improving diffusion-based RL methods for the subsequent works.
% % \todo{the base diffusion distribution} towards high-return \todo{areas}.
% (\romannumeral 2) We perform contrastive learning over returns of states to improve the base distribution. To the best of our knowledge, our work is the first which notices the limitation of the base distribution, and the first which applies contrastive learning to enhance the base distribution for diffusion based RL methods.
% (\romannumeral 3) Experiment results on 14 D4RL datasets demonstrate the outstanding performance of CDiffuser.
% , as well as the success of the guided \todo{ base distribution} learning provided by contrastive learning.

% adopts contrastive learning and is capable of generating biased trajectories towards the area of higher return states. (3) Experiments on D4RL datasets show that CDiffuser outperforms other baseline methods and further demonstrates the significance of the \textit{state-return} distribution in successful action prediction. (4) Thanks to the consideration of the \textit{state-return} distribution, CDiffuser is able to mitigate the out-of-distribution (OOD) problem as it intentionally encourages the agent to approach the high-potential state distribution, which is precisely in the distribution of collected dataset. 

% Noticing the aforementioned challenges while inspired by contrastive learning, we propose \textbf{CDiffuser}, which pays attention on $state-return$ distribution and adopt contrastive learning to bias the learning process towards high-return states while away from low-return states, thus guides the learning of trajectory generation and leverages the information present in the dataset more comprehensively.
% Specifically, we adopt a trajectory generation model based on diffusion models as the base model, while an auxiliary optimize object based on contrastive learning is further adopted to ensure that the predicted trajectories' states fall within the positive sample distribution as much as possible while avoiding the negative sample distribution. 
% Details of our model will be further detailed in \cref{sec:Methods}. Experiment results on nine commonly used benchmarks demonstrates that CDiffuser has the capability to guide the agent towards a state space characterized by higher returns, thus exhibiting superior performance compared to existing methods.

% In summary, our contributions are as follows: (1) We identify the shortcomings of existing diffusion-based RL methods and provide a practical solution. (2) We propose a novel diffusion-based RL method, CDiffuser, which adopts contrastive learning and is capable of generating biased trajectories towards the area of higher return states. (3) Experiments on D4RL datasets show that CDiffuser outperforms other baseline methods and further demonstrates the significance of the \textit{state-return} distribution in successful action prediction. (4) Thanks to the consideration of the \textit{state-return} distribution, CDiffuser is able to mitigate the out-of-distribution (OOD) problem as it intentionally encourages the agent to approach the high-potential state distribution, which is precisely in the distribution of collected dataset. 


==> papers/checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The main claims made in the abstract and introduction accurately reflect the paper's contributions and scope, and the contributions of our work are listed in \cref{sec:intro}. The experimental results have validated our standpoint and also demonstrated the effectiveness of the proposed method.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have discussed the limitations and future works of CDiffuser in \cref{conclusion}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not include theoretical results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We displayed the model structure in \cref{fig:framework} and elaborated on the details of the CDiffuser model in \cref{sec:Methods}. We have also provide the pseudo code of CDiffuser in \cref{appendix:cluster}, \cref{appendix:psuedo:planning} and \cref{appendix:psuedo:train}. Our code is publicly available at anonymous link \url{https://anonymous.4open.science/r/CDiffuser}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The code, instructions and dataset links are publicly available at anonymous link \url{https://anonymous.4open.science/r/CDiffuser}. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All the training and test details are detailed in \cref{sec:exp}. We have also discussed how to select two types of our proposed model in \cref{appendix:choice}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have reported the error bars suitably and correctly in our experiments, specififcally in \cref{tab:data}, \cref{tab:data-mix}, \cref{tab:cdd} and \cref{tab:all:mix}. The error bars are reported as standard deviations evaluated on various seeds, denoted with $\pm$.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provided a detailed report on our experimental environment in \cref{sec:resource}, including the GPU model and quantity, CPU model and core count, and memory usage.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have thoroughly reviewed the the NeurIPS Code of Ethics, and have ensured the compliance of our work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work will not cause any direct positive or negative social impacts.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our models does not have a high risk for misuse or risky dual-usage.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We confirm that all the codes, data, or models used in the paper are credited, and the license and terms of use explicitly mentioned and properly respected.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All of the code, data, models in the paper are provided at anonymous link \url{https://anonymous.4open.science/r/CDiffuser} along with the instructions. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  Our paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

